Attention Guided Graph Convolutional Networks for Relation Extraction

Dependency trees convey rich structural information that is proven useful for extracting relations among entities in text. However, how to effectively make use of relevant information while ignoring irrelevant information from the dependency trees remains a challenging research question. Existing approaches employing rule based hard-pruning strategies for selecting relevant partial dependency structures may not always yield optimal results. In this work, we propose Attention Guided Graph Convolutional Networks (AGGCNs), a novel model which directly takes full dependency trees as inputs. Our model can be understood as a soft-pruning approach that automatically learns how to selectively attend to the relevant sub-structures useful for the relation extraction task. Extensive results on various tasks including cross-sentence n-ary relation extraction and large-scale sentence-level relation extraction show that our model is able to better leverage the structural information of the full dependency trees, giving significantly better results than previous approaches.

==> Attention Guided Graph Convolutional Networks for Relation Extraction (Arxiv)/table/table1.tex <==
\begin{table*}[!th]
% \small
\centering
\setlength{\tabcolsep}{2.5pt}
\scalebox{0.9}{
\begin{tabular}{lcccccccc} 
\toprule
    \multirow{3}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Binary-class}} & \multicolumn{2}{c}{\textbf{Multi-class}} \\
\cmidrule(l{5pt}r{5pt}){2-5} \cmidrule(l{5pt}r{5pt}){6-7}
    & \multicolumn{2}{c}{T} & \multicolumn{2}{c}{B}  & T & B\\
% \cmidrule(l{5pt}r{5pt}){2-3} \cmidrule(l{5pt}r{5pt}){4-5}
& \texttt{Single} & \texttt{Cross} & \texttt{Single} & \texttt{Cross} & \texttt{Cross} & \texttt{Cross}  \\
\midrule
Feature-Based~\citep{Quirk2017DistantSF}        & 74.7 & 77.7 & 73.9 & 75.2  &- & -\\
SPTree~\citep{Miwa2016EndtoEndRE}            &  -   & -    &75.9  & 75.9  &- & -\\
Graph LSTM-EMBED~\citep{Peng2017CrossSentenceNR}& 76.5 & 80.6 &74.3  & 76.5 &- & -\\
Graph LSTM-FULL~\citep{Peng2017CrossSentenceNR} & 77.9 &80.7  &75.6  & 76.7 &- & -\\
{\color{white}00000000000000000} + multi-task                      & -    &  82.0  & -  & 78.5 &- & -\\
Bidir DAG LSTM~\citep{Song2018NaryRE}           & 75.6 & 77.3 &76.9  & 76.4    & 51.7 &	50.7\\
GS GLSTM~\citep{Song2018NaryRE}                 & 80.3 & 83.2 &83.5  & 83.6    & 71.7 &	71.7 \\
\midrule
GCN (Full Tree)~\citep{Zhang2018GraphCO}                                   &84.3 &84.8 & 84.2 & 83.6 & 77.5  &	74.3\\
GCN ($K$=0)~\citep{Zhang2018GraphCO}                                             &85.8    &85.8 & 82.8 & 82.7 & 75.6  &	72.3\\
GCN ($K$=1)~\citep{Zhang2018GraphCO}                                        &85.4    &85.7   & 83.5 & 83.4 & 78.1  &	73.6\\
GCN ($K$=2)~\citep{Zhang2018GraphCO}                                        &84.7    &85.0   & 83.8 & 83.7 & 77.9  &	73.1\\
\midrule
AGGCN (ours)                                     & \textbf{87.1} & \textbf{87.0} & \textbf{85.2} & \textbf{85.6}  & \textbf{79.7} &  \textbf{77.4}\\
\bottomrule
\end{tabular}}
% \vspace{-1mm}
\caption{Average test accuracies in five-fold validation for binary-class $n$-ary relation extraction and multi-class $n$-ary relation extraction.  ``T'' and  ``B'' denote ternary drug-gene-mutation interactions and binary drug-mutation interactions, respectively.  \texttt{Single} means that we report the accuracy on instances within single sentences, while \texttt{Cross} means the accuracy on all instances. $K$ in the GCN models means that the preprocessed pruned trees include tokens up to distance $K$ away from the dependency path in the  LCA subtree.}
\vspace{-3mm}
\label{tab:tern_bin}
\end{table*}


==> Attention Guided Graph Convolutional Networks for Relation Extraction (Arxiv)/table/table2.tex <==

\begin{table}[!t]
% 	\small
	\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcc}
\toprule
\bf Model & Ternary & Binary \\
\midrule
Bidir DAG LSTM~\citep{Song2018NaryRE} & 51.7 &	50.7 \\
GS GLSTM~\citep{Song2018NaryRE}       & 71.7 &	71.7 \\
\midrule
GCN (Full Tree)~\citep{Zhang2018GraphCO}          & 77.5  &	74.3 \\
GCN (K=0)~\citep{Zhang2018GraphCO}          & 75.6  &	72.3 \\
GCN (K=1)~\citep{Zhang2018GraphCO}     & 78.1  &	73.6 \\
GCN (K=2)~\citep{Zhang2018GraphCO}     & 77.9  &	73.1 \\
\midrule
AGGCN (ours)                            & \textbf{79.7} &  \textbf{77.4} \\
\bottomrule
\end{tabular}
% \vspace{-1mm}
\caption{Average test accuracies for multi-class relation extraction on all instances (\texttt{Cross}). }
% \vspace{-1mm}
\label{tab:multi-class}
\end{table}



==> Attention Guided Graph Convolutional Networks for Relation Extraction (Arxiv)/table/table3.tex <==
\begin{table}[!t]
% 	\small
	\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
\bf Model & P & R & F1 \\
\midrule
LR~\citep{Zhang2017PositionawareAA}          & \textbf{73.5} &49.9 &	59.4 \\
SDP-LSTM~\citep{Xu2015ClassifyingRV}{*}    & 66.3 &52.7 &	58.7 \\
Tree-LSTM~\citep{Tai2015ImprovedSR}{**}          & 66.0 &59.2 &	62.4\\
PA-LSTM~\citep{Zhang2017PositionawareAA}     & 65.7 & \textbf{64.5} &	65.1\\
\midrule
GCN~\citep{Zhang2018GraphCO}                 & 69.8 &59.0 &	64.0\\
C-GCN~\citep{Zhang2018GraphCO}               & 69.9 &63.3 &	66.4\\
\midrule
AGGCN (ours)                                 & 69.9 & 60.9 &	65.1 \\
C-AGGCN (ours)                            & 73.1 & 64.2  & \textbf{69.0} \\
\bottomrule
\end{tabular}
% \vspace{-1mm}
\caption{Results on the TACRED dataset. Model with * indicates that the results are reported in~\citet{Zhang2017PositionawareAA}, while model with ** indicates the results are reported in~\citet{Zhang2018GraphCO}.  Our model with default random seed (0) achieves 69.0 F1 score. {The trained model is available for download, together with code and other details for reproducing the results. Following other practices in the community, we also conducted further experiments with 4 additional random seeds, and the averaged result over the 5 runs was: mean F1 68.2 with standard deviation 0.5.}}
\label{tab:tacred}
\end{table}


==> Attention Guided Graph Convolutional Networks for Relation Extraction (Arxiv)/table/table4.tex <==
\begin{table}[!t]
% 	\small
	\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcccc}
\toprule
\bf Model & & & &F1 \\
\midrule
SVM~\citep{Rink2010UTDCS}               & & & & 82.2\\
SDP-LSTM~\citep{Xu2015ClassifyingRV}    & & & & 83.7\\
SPTree~\citep{Miwa2016EndtoEndRE}       & & & & 84.4\\
PA-LSTM~\citep{Zhang2017PositionawareAA}& & & & 82.7\\
C-GCN~\citep{Zhang2018GraphCO}          & & & & 84.8\\
\midrule
C-AGGCN (ours)                           & & & &\textbf{85.7}    \\
\bottomrule
\end{tabular}
% \vspace{-2mm}
\caption{Results on the SemEval dataset. }
% \vspace{-4mm}
\label{tab:semeval}
\end{table}




==> Attention Guided Graph Convolutional Networks for Relation Extraction (Arxiv)/table/table5.tex <==
\begin{table}[!t]
% 	\small
	\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcccc}
\toprule
\bf Model & & & &F1 \\
\midrule
C-AGGCN              & & & & 69.0\\
{\color{white}0}   -- Attention-guided layer (AG) &  & & & 67.1\\
{\color{white}0}   -- Dense connected layer (DC)  &  & & & 67.3 \\
{\color{white}0}   -- AG, DC   &  & & &66.7\\
{\color{white}0}   -- Feed-Forward layer (FF)    &  & & & 67.8\\
% {\color{white}0}   -- Multi-head attention    &  & & &66.9\\
\bottomrule
\end{tabular}
% \vspace{-2mm}
\caption{An ablation study for C-AGGCN model. }
% \vspace{-1mm}
\label{tab:ablation}
\end{table}



==> Attention Guided Graph Convolutional Networks for Relation Extraction (Arxiv)/table/table6.tex <==
\begin{table}[!t]
% 	\small
	\centering
\setlength{\tabcolsep}{3pt}
% \captionsetup{justification=centering,margin=0.25cm}
\begin{tabular}{lcccc}
\toprule
\bf Model & & & &F1 \\
\midrule
C-AGGCN (Full tree)             & & & & 69.0\\
C-AGGCN ($K$=2)             & & & & 67.5\\
C-AGGCN ($K$=1)             & & & & 67.9\\
C-AGGCN ($K$=0)             & & & & 67.0\\
\bottomrule
\end{tabular}
% \vspace{-2mm}
\caption{Results of C-AGGCN with pruned trees.}
% \vspace{-3mm}
\label{tab:prune_tree}
\end{table}



==> table/table2.tex <==

\begin{table}[!t]
% 	\small
	\centering
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lcc}
\toprule
\bf Model & Ternary & Binary \\
\midrule
Bidir DAG LSTM~\citep{Song2018NaryRE} & 51.7 &	50.7 \\
GS GLSTM~\citep{Song2018NaryRE}       & 71.7 &	71.7 \\
\midrule
GCN (Full Tree)~\citep{Zhang2018GraphCO}          & 77.5  &	74.3 \\
GCN (K=0)~\citep{Zhang2018GraphCO}          & 75.6  &	72.3 \\
GCN (K=1)~\citep{Zhang2018GraphCO}     & 78.1  &	73.6 \\
GCN (K=2)~\citep{Zhang2018GraphCO}     & 77.9  &	73.1 \\
\midrule
AGGCN (ours)                            & \textbf{79.7} &  \textbf{77.4} \\
\bottomrule
\end{tabular}
% \vspace{-1mm}
\caption{Average test accuracies for multi-class relation extraction on all instances (\texttt{Cross}). }
% \vspace{-1mm}
\label{tab:multi-class}
\end{table}


